Translocation and encapsulation of siRNA inside carbon nanotubes

We report spontaneous translocation of small interfering RNA (siRNA) inside carbon nanotubes (CNTs) of various diameters and chirality using all atom molecular dynamics (MD) simulations with explicit solvent. We use Umbrella sampling method to calculate the free energy landscape of the siRNA entry and translocation event. Free energy profiles shows that siRNA gains free energy while translocating inside CNT and barrier for siRNA exit from CNT ranges from 40 to 110 kcal/mol depending on CNT chirality and salt concentration. The translocation time \tau decreases with the increase of CNT diameter with a critical diameter of 24 \AA for the translocation. In contrast, double strand DNA (dsDNA) of the same sequence does not translocate inside CNT due to large free energy barrier for the translocation. This study helps in understanding the nucleic acid transport through nanopores at microscopic level and may help designing carbon nanotube based sensor for siRNA.

==> run_sh <==
#!/bin/bash
for i in *eps; do ps2pdf -DEPSCrop $i; done
#sed -i 's/\.eps}/}/g' *tex

